Block Palindromes: A New Generalization of Palindromes

We study a new generalization of palindromes and gapped palindromes called block palindromes. A block palindrome is a string that becomes a palindrome when identical substrings are replaced with a distinct character. We investigate several properties of block palindromes and in particular, study substrings of a string which are block palindromes. In so doing, we introduce the notion of a \emph{maximal block palindrome}, which leads to a compact representation of all block palindromes that occur in a string. We also propose an algorithm which enumerates all maximal block palindromes that appear in a given string $T$ in $O(|T| + \|\mathit{MBP}(T)\|)$ time, where $\|\mathit{MBP}(T)\|$ is the output size, which is optimal unless all the maximal block palindromes can be represented in a more compact way.

==> texdir/macro-color.tex <==
\usepackage[whole]{bxcjkjatype}

% Basic
\definecolor{color555428}{rgb}{0.52,0.67,0.92} \newcommand{\T}{{\setlength{\fboxsep}{0pt}\colorbox{color555428}{$T$}}}

% Alphabet
%\newcommand{\aa}{a} % already defined
\definecolor{color152165}{rgb}{0.41,0.40,0.82} \newcommand{\bb}{{\setlength{\fboxsep}{0pt}\colorbox{color152165}{$b$}}}
\definecolor{color756842}{rgb}{0.43,0.69,0.57} \newcommand{\cc}{{\setlength{\fboxsep}{0pt}\colorbox{color756842}{$c$}}}
\definecolor{color376495}{rgb}{0.98,0.70,0.86} \newcommand{\dd}{{\setlength{\fboxsep}{0pt}\colorbox{color376495}{$d$}}}
\definecolor{color412927}{rgb}{0.87,0.72,0.73} \newcommand{\ee}{{\setlength{\fboxsep}{0pt}\colorbox{color412927}{$e$}}}
\definecolor{color587028}{rgb}{0.98,0.82,0.60} \newcommand{\ff}{{\setlength{\fboxsep}{0pt}\colorbox{color587028}{$f$}}}
%\newcommand{\gg}{g} % already defined
\definecolor{color294163}{rgb}{0.87,1.00,0.47} \newcommand{\hh}{{\setlength{\fboxsep}{0pt}\colorbox{color294163}{$h$}}}
\definecolor{color703852}{rgb}{0.99,0.94,0.72} \newcommand{\ii}{{\setlength{\fboxsep}{0pt}\colorbox{color703852}{$i$}}}
\definecolor{color798822}{rgb}{0.63,0.62,0.63} \newcommand{\jj}{{\setlength{\fboxsep}{0pt}\colorbox{color798822}{$j$}}}
\definecolor{color201266}{rgb}{0.55,0.57,0.51} \newcommand{\kk}{{\setlength{\fboxsep}{0pt}\colorbox{color201266}{$k$}}}
%\newcommand{\ll}{l} % already defined
\definecolor{color673344}{rgb}{0.95,0.53,0.57} \newcommand{\mm}{{\setlength{\fboxsep}{0pt}\colorbox{color673344}{$m$}}}
\definecolor{color527264}{rgb}{0.76,0.51,0.66} \newcommand{\nn}{{\setlength{\fboxsep}{0pt}\colorbox{color527264}{$n$}}}
\definecolor{color855462}{rgb}{0.68,0.87,0.87} \newcommand{\oo}{{\setlength{\fboxsep}{0pt}\colorbox{color855462}{$o$}}}
\definecolor{color426550}{rgb}{0.46,0.72,0.62} \newcommand{\pp}{{\setlength{\fboxsep}{0pt}\colorbox{color426550}{$p$}}}
\definecolor{color531436}{rgb}{0.98,0.97,0.83} \newcommand{\qq}{{\setlength{\fboxsep}{0pt}\colorbox{color531436}{$q$}}}
\definecolor{color394989}{rgb}{0.96,0.66,0.73} \newcommand{\rr}{{\setlength{\fboxsep}{0pt}\colorbox{color394989}{$r$}}}
%\newcommand{\ss}{s} % already defined
%\newcommand{\tt}{t} % already defined
\definecolor{color383718}{rgb}{0.99,0.86,0.53} \newcommand{\uu}{{\setlength{\fboxsep}{0pt}\colorbox{color383718}{$u$}}}
%\definecolor{color230651}{rgb}{0.78,0.53,0.70} \newcommand{\vv}{{\setlength{\fboxsep}{0pt}\colorbox{color230651}{$v$}}}
\definecolor{color961079}{rgb}{0.41,0.50,0.95} \newcommand{\ww}{{\setlength{\fboxsep}{0pt}\colorbox{color961079}{$w$}}}
\definecolor{color93733}{rgb}{0.61,0.55,0.89} \newcommand{\xx}{{\setlength{\fboxsep}{0pt}\colorbox{color93733}{$x$}}}
\definecolor{color433286}{rgb}{0.73,0.56,0.68} \newcommand{\yy}{{\setlength{\fboxsep}{0pt}\colorbox{color433286}{$y$}}}
\definecolor{color665096}{rgb}{0.83,0.90,0.77} \newcommand{\zz}{{\setlength{\fboxsep}{0pt}\colorbox{color665096}{$z$}}}

%\newcommand{\AA}{A} % already defined
\definecolor{color94056}{rgb}{0.40,0.82,0.89} \newcommand{\BB}{{\setlength{\fboxsep}{0pt}\colorbox{color94056}{$B$}}}
\definecolor{color564494}{rgb}{0.90,0.96,0.95} \newcommand{\CC}{{\setlength{\fboxsep}{0pt}\colorbox{color564494}{$C$}}}
\definecolor{color361279}{rgb}{0.40,0.90,0.60} \newcommand{\DD}{{\setlength{\fboxsep}{0pt}\colorbox{color361279}{$D$}}}
\definecolor{color787561}{rgb}{0.48,0.80,0.41} \newcommand{\EE}{{\setlength{\fboxsep}{0pt}\colorbox{color787561}{$E$}}}
\definecolor{color861901}{rgb}{0.83,0.52,0.99} \newcommand{\FF}{{\setlength{\fboxsep}{0pt}\colorbox{color861901}{$F$}}}
\definecolor{color199437}{rgb}{0.59,0.96,0.93} \newcommand{\GG}{{\setlength{\fboxsep}{0pt}\colorbox{color199437}{$G$}}}
\definecolor{color929869}{rgb}{0.92,0.75,0.42} \newcommand{\HH}{{\setlength{\fboxsep}{0pt}\colorbox{color929869}{$H$}}}
\definecolor{color102290}{rgb}{0.44,0.96,0.40} \newcommand{\II}{{\setlength{\fboxsep}{0pt}\colorbox{color102290}{$I$}}}
\definecolor{color240502}{rgb}{0.98,0.98,0.75} \newcommand{\JJ}{{\setlength{\fboxsep}{0pt}\colorbox{color240502}{$J$}}}
\definecolor{color528764}{rgb}{0.80,0.75,0.40} \newcommand{\KK}{{\setlength{\fboxsep}{0pt}\colorbox{color528764}{$K$}}}
\definecolor{color149897}{rgb}{0.60,0.41,0.47} \newcommand{\LL}{{\setlength{\fboxsep}{0pt}\colorbox{color149897}{$L$}}}
\definecolor{color28559}{rgb}{0.56,0.41,0.91} \newcommand{\MM}{{\setlength{\fboxsep}{0pt}\colorbox{color28559}{$M$}}}
\definecolor{color342219}{rgb}{0.72,0.81,0.56} \newcommand{\NN}{{\setlength{\fboxsep}{0pt}\colorbox{color342219}{$N$}}}
\definecolor{color43484}{rgb}{0.78,0.61,0.60} \newcommand{\OO}{{\setlength{\fboxsep}{0pt}\colorbox{color43484}{$O$}}}
\definecolor{color906068}{rgb}{0.40,0.90,0.81} \newcommand{\PP}{{\setlength{\fboxsep}{0pt}\colorbox{color906068}{$P$}}}
\definecolor{color819975}{rgb}{0.45,0.96,0.89} \newcommand{\QQ}{{\setlength{\fboxsep}{0pt}\colorbox{color819975}{$Q$}}}
\definecolor{color867690}{rgb}{0.56,0.69,0.54} \newcommand{\RR}{{\setlength{\fboxsep}{0pt}\colorbox{color867690}{$R$}}}
%\newcommand{\SS}{S} % already defined
\definecolor{color958062}{rgb}{0.85,0.58,0.98} \newcommand{\TT}{{\setlength{\fboxsep}{0pt}\colorbox{color958062}{$T$}}}
\definecolor{color566600}{rgb}{0.93,0.64,0.70} \newcommand{\UU}{{\setlength{\fboxsep}{0pt}\colorbox{color566600}{$U$}}}
\definecolor{color214332}{rgb}{0.62,0.69,0.72} \newcommand{\VV}{{\setlength{\fboxsep}{0pt}\colorbox{color214332}{$V$}}}
\definecolor{color481108}{rgb}{0.48,0.98,0.53} \newcommand{\WW}{{\setlength{\fboxsep}{0pt}\colorbox{color481108}{$W$}}}
\definecolor{color266789}{rgb}{0.67,0.46,0.56} \newcommand{\XX}{{\setlength{\fboxsep}{0pt}\colorbox{color266789}{$X$}}}
\definecolor{color548485}{rgb}{0.87,0.81,0.76} \newcommand{\YY}{{\setlength{\fboxsep}{0pt}\colorbox{color548485}{$Y$}}}
\definecolor{color385402}{rgb}{0.55,0.91,0.56} \newcommand{\ZZ}{{\setlength{\fboxsep}{0pt}\colorbox{color385402}{$Z$}}}

% prefixed with v
\definecolor{color741973}{rgb}{0.90,0.44,0.73} \newcommand{\va}{{\setlength{\fboxsep}{0pt}\colorbox{color741973}{$a$}}}
\definecolor{color613860}{rgb}{0.64,0.77,0.98} \newcommand{\vb}{{\setlength{\fboxsep}{0pt}\colorbox{color613860}{$b$}}}
\definecolor{color473389}{rgb}{0.80,0.40,0.91} \newcommand{\vc}{{\setlength{\fboxsep}{0pt}\colorbox{color473389}{$c$}}}
\definecolor{color101268}{rgb}{0.85,0.69,0.85} \newcommand{\vd}{{\setlength{\fboxsep}{0pt}\colorbox{color101268}{$d$}}}
\definecolor{color573610}{rgb}{0.62,0.55,0.90} \newcommand{\ve}{{\setlength{\fboxsep}{0pt}\colorbox{color573610}{$e$}}}
\definecolor{color509810}{rgb}{0.70,0.51,0.62} \newcommand{\vf}{{\setlength{\fboxsep}{0pt}\colorbox{color509810}{$f$}}}
\definecolor{color675636}{rgb}{0.67,0.79,0.49} \newcommand{\vg}{{\setlength{\fboxsep}{0pt}\colorbox{color675636}{$g$}}}
\definecolor{color131282}{rgb}{0.55,0.98,0.41} \newcommand{\vh}{{\setlength{\fboxsep}{0pt}\colorbox{color131282}{$h$}}}
\definecolor{color674619}{rgb}{0.72,0.96,0.83} \newcommand{\vi}{{\setlength{\fboxsep}{0pt}\colorbox{color674619}{$i$}}}
\definecolor{color569168}{rgb}{0.73,0.95,0.55} \newcommand{\vj}{{\setlength{\fboxsep}{0pt}\colorbox{color569168}{$j$}}}
\definecolor{color906491}{rgb}{0.55,0.40,0.76} \newcommand{\vk}{{\setlength{\fboxsep}{0pt}\colorbox{color906491}{$k$}}}
\definecolor{color188778}{rgb}{0.64,0.78,0.89} \newcommand{\vl}{{\setlength{\fboxsep}{0pt}\colorbox{color188778}{$l$}}}
\definecolor{color922655}{rgb}{0.70,0.77,0.96} \newcommand{\vm}{{\setlength{\fboxsep}{0pt}\colorbox{color922655}{$m$}}}
\definecolor{color744995}{rgb}{0.91,0.40,0.62} \newcommand{\vn}{{\setlength{\fboxsep}{0pt}\colorbox{color744995}{$n$}}}
\definecolor{color756106}{rgb}{0.93,0.41,0.93} \newcommand{\vo}{{\setlength{\fboxsep}{0pt}\colorbox{color756106}{$o$}}}
\definecolor{color38845}{rgb}{0.76,0.99,0.93} \newcommand{\vp}{{\setlength{\fboxsep}{0pt}\colorbox{color38845}{$p$}}}
\definecolor{color247546}{rgb}{0.96,0.56,0.55} \newcommand{\vq}{{\setlength{\fboxsep}{0pt}\colorbox{color247546}{$q$}}}
\definecolor{color808062}{rgb}{0.70,0.51,0.71} \newcommand{\vr}{{\setlength{\fboxsep}{0pt}\colorbox{color808062}{$r$}}}
\definecolor{color124589}{rgb}{0.49,0.95,0.68} \newcommand{\vs}{{\setlength{\fboxsep}{0pt}\colorbox{color124589}{$s$}}}
\definecolor{color683898}{rgb}{0.58,0.43,0.44} \newcommand{\vt}{{\setlength{\fboxsep}{0pt}\colorbox{color683898}{$t$}}}
\definecolor{color330519}{rgb}{0.94,0.62,0.62} \newcommand{\vu}{{\setlength{\fboxsep}{0pt}\colorbox{color330519}{$u$}}}
\definecolor{color358725}{rgb}{0.87,0.65,0.78} \newcommand{\vv}{{\setlength{\fboxsep}{0pt}\colorbox{color358725}{$v$}}}
\definecolor{color882109}{rgb}{0.61,0.83,0.69} \newcommand{\vw}{{\setlength{\fboxsep}{0pt}\colorbox{color882109}{$w$}}}
\definecolor{color391609}{rgb}{0.71,0.54,0.56} \newcommand{\vx}{{\setlength{\fboxsep}{0pt}\colorbox{color391609}{$x$}}}
\definecolor{color172178}{rgb}{0.79,0.93,0.77} \newcommand{\vy}{{\setlength{\fboxsep}{0pt}\colorbox{color172178}{$y$}}}
\definecolor{color946281}{rgb}{0.87,0.77,0.69} \newcommand{\vz}{{\setlength{\fboxsep}{0pt}\colorbox{color946281}{$z$}}}

\definecolor{color332076}{rgb}{0.53,0.41,0.82} \newcommand{\vA}{{\setlength{\fboxsep}{0pt}\colorbox{color332076}{$A$}}}
\definecolor{color602878}{rgb}{0.49,0.97,0.51} \newcommand{\vB}{{\setlength{\fboxsep}{0pt}\colorbox{color602878}{$B$}}}
\definecolor{color785183}{rgb}{0.64,0.84,0.47} \newcommand{\vC}{{\setlength{\fboxsep}{0pt}\colorbox{color785183}{$C$}}}
\definecolor{color776441}{rgb}{0.51,0.67,0.58} \newcommand{\vD}{{\setlength{\fboxsep}{0pt}\colorbox{color776441}{$D$}}}
\definecolor{color180676}{rgb}{0.77,0.69,0.89} \newcommand{\vE}{{\setlength{\fboxsep}{0pt}\colorbox{color180676}{$E$}}}
\definecolor{color198513}{rgb}{0.69,0.62,0.70} \newcommand{\vF}{{\setlength{\fboxsep}{0pt}\colorbox{color198513}{$F$}}}
\definecolor{color12131}{rgb}{0.47,0.61,0.54} \newcommand{\vG}{{\setlength{\fboxsep}{0pt}\colorbox{color12131}{$G$}}}
\definecolor{color196862}{rgb}{0.85,0.68,0.98} \newcommand{\vH}{{\setlength{\fboxsep}{0pt}\colorbox{color196862}{$H$}}}
\definecolor{color450969}{rgb}{0.47,0.83,0.98} \newcommand{\vI}{{\setlength{\fboxsep}{0pt}\colorbox{color450969}{$I$}}}
\definecolor{color67393}{rgb}{0.63,0.71,0.69} \newcommand{\vJ}{{\setlength{\fboxsep}{0pt}\colorbox{color67393}{$J$}}}
\definecolor{color847675}{rgb}{0.81,0.73,0.97} \newcommand{\vK}{{\setlength{\fboxsep}{0pt}\colorbox{color847675}{$K$}}}
\definecolor{color170629}{rgb}{0.67,0.71,0.87} \newcommand{\vL}{{\setlength{\fboxsep}{0pt}\colorbox{color170629}{$L$}}}
\definecolor{color75747}{rgb}{0.71,0.61,0.77} \newcommand{\vM}{{\setlength{\fboxsep}{0pt}\colorbox{color75747}{$M$}}}
\definecolor{color922298}{rgb}{0.81,0.58,0.45} \newcommand{\vN}{{\setlength{\fboxsep}{0pt}\colorbox{color922298}{$N$}}}
\definecolor{color461222}{rgb}{0.77,0.90,0.71} \newcommand{\vO}{{\setlength{\fboxsep}{0pt}\colorbox{color461222}{$O$}}}
\definecolor{color842162}{rgb}{0.98,0.94,0.46} \newcommand{\vP}{{\setlength{\fboxsep}{0pt}\colorbox{color842162}{$P$}}}
\definecolor{color40271}{rgb}{0.50,0.46,0.80} \newcommand{\vQ}{{\setlength{\fboxsep}{0pt}\colorbox{color40271}{$Q$}}}
\definecolor{color508723}{rgb}{0.59,0.55,0.75} \newcommand{\vR}{{\setlength{\fboxsep}{0pt}\colorbox{color508723}{$R$}}}
\definecolor{color54698}{rgb}{0.73,0.40,0.86} \newcommand{\vS}{{\setlength{\fboxsep}{0pt}\colorbox{color54698}{$S$}}}
\definecolor{color145077}{rgb}{0.55,0.83,0.90} \newcommand{\vT}{{\setlength{\fboxsep}{0pt}\colorbox{color145077}{$T$}}}
\definecolor{color2201}{rgb}{0.46,0.43,0.47} \newcommand{\vU}{{\setlength{\fboxsep}{0pt}\colorbox{color2201}{$U$}}}
\definecolor{color360647}{rgb}{0.59,0.98,0.80} \newcommand{\vV}{{\setlength{\fboxsep}{0pt}\colorbox{color360647}{$V$}}}
\definecolor{color999517}{rgb}{0.65,0.53,0.73} \newcommand{\vW}{{\setlength{\fboxsep}{0pt}\colorbox{color999517}{$W$}}}
\definecolor{color403460}{rgb}{0.72,0.41,0.49} \newcommand{\vX}{{\setlength{\fboxsep}{0pt}\colorbox{color403460}{$X$}}}
\definecolor{color983403}{rgb}{0.58,0.58,0.67} \newcommand{\vY}{{\setlength{\fboxsep}{0pt}\colorbox{color983403}{$Y$}}}
\definecolor{color222935}{rgb}{0.55,0.93,0.78} \newcommand{\vZ}{{\setlength{\fboxsep}{0pt}\colorbox{color222935}{$Z$}}}


% Function
\definecolor{color920695}{rgb}{0.41,0.73,0.84} \newcommand{\floor}[1]{{\setlength{\fboxsep}{0pt}\colorbox{color920695}{$\lfloor #1 \rfloor$}}}
\definecolor{color757318}{rgb}{0.71,0.50,0.43} \newcommand{\ceil}[1]{{\setlength{\fboxsep}{0pt}\colorbox{color757318}{$\lceil #1 \rceil$}}}
\definecolor{color55687}{rgb}{0.44,0.67,0.80} \newcommand{\LCE}{{\setlength{\fboxsep}{0pt}\colorbox{color55687}{$LCE$}}}

\newcommand{\attention}[1]{\textcolor{red}{[#1]}}

% For this paper
\definecolor{color660912}{rgb}{0.43,0.58,0.52} \newcommand{\bpos}[1]{{\setlength{\fboxsep}{0pt}\colorbox{color660912}{$b(#1)$}}}
\definecolor{color729260}{rgb}{0.94,0.89,0.62} \newcommand{\epos}[1]{{\setlength{\fboxsep}{0pt}\colorbox{color729260}{$e(#1)$}}}
\newcommand{\MBP}{\mathit{MBP}}
\newcommand{\occ}{\mathit{occ}}
\newcommand{\bocc}{\mathit{occUB}}
\newcommand{\blen}{\mathit{blen}}

%\definecolor{color848673}{rgb}{0.60,0.94,0.78} \newcommand{\bp}{{\setlength{\fboxsep}{0pt}\colorbox{color848673}{$block palindrome\xspace$}}}

